On the Complexity of Computing Minimal Unsatisfiable LTL formulas

We show that (1) the Minimal False QCNF search-problem (MF-search) and the Minimal Unsatisfiable LTL formula search problem (MU-search) are FPSPACE complete because of the very expressive power of QBF/LTL, (2) we extend the PSPACE-hardness of the MF decision problem to the MU decision problem. As a consequence, we deduce a positive answer to the open question of PSPACE hardness of the inherent Vacuity Checking problem. We even show that the Inherent Non Vacuous formula search problem is also FPSPACE-complete.

==> paperorganisation.tex <==
 For uniformity purpose we introduce QLTL ($QBF \subset QLTL$ and $LTL \subset QLTL$) in   Section 2.  Section 3 discusses the notions of weakening for QLTL formulas and minimal unsatisfiable LTL formulas.  In Section 4,  we present other LTL causes based problems and show how to reduce them to  causes based problems of LTL unsatisfiability. In section 5, we start by  analyzing the complexity of Minimal FALSE QCNF formulas, then, we enhance the translation of QCNF sat  to LTL Model Checking to show complexity results for some causes based problems in models and for the LTL MU-search problem. Finally, we  propose an original proof of PSPACE completeness of the MU-dec problem and  we reuse this result in order to provide complexity result for Inherent Vacuity Checking. We conclude in Section 6. An appendix contains acronyms, the details of definitions of some causes based problems, the schema of the reductions and details of the proofs. %  A full  paper is available at http://liris.cnrs.fr/$\sim$fhantry/

